Photorealistic Style Transfer with Screened Poisson Equation

Recent work has shown impressive success in transferring painterly style to images. These approaches, however, fall short of photorealistic style transfer. Even when both the input and reference images are photographs, the output still exhibits distortions reminiscent of a painting. In this paper we propose an approach that takes as input a stylized image and makes it more photorealistic. It relies on the Screened Poisson Equation, maintaining the fidelity of the stylized image while constraining the gradients to those of the original input image. Our method is fast, simple, fully automatic and shows positive progress in making a stylized image photorealistic. Our results exhibit finer details and are less prone to artifacts than the state-of-the-art.

==> fig_compare_wu.tex <==
\begin{figure}
		\centering
        \setlength{\tabcolsep}{.15em}
        \small
        \begin{tabular}{cc|ccc} 
		\includegraphics[width=.19\linewidth]{wu/in13.png}&
		\includegraphics[width=.19\linewidth]{wu/tar13.png}&
		\includegraphics[width=.19\linewidth]{wu/wu13.png}&
        \includegraphics[width=.19\linewidth]{wu/NS_seg_13.png}&
		\includegraphics[width=.19\linewidth]{wu/out13.png}\\
		\includegraphics[width=.19\linewidth]{wu/in3.png}&
		\includegraphics[width=.19\linewidth]{wu/tar3.png}&
        \includegraphics[width=.19\linewidth]{wu/wu3.png}&
        \includegraphics[width=.19\linewidth]{wu/NS_seg_3.png}&
		\includegraphics[width=.19\linewidth]{wu/out3.png}\\
        Input image& Style image& Wu et al.~\cite{wu2013content}& NeuralStyle+SPE& StyleSwap+SPE\\
        \end{tabular}
		\caption{Comparison with Wu et al.~\cite{wu2013content} content-aware color transfer method, although produce nice results it fails when the semantic information is missing -- see the bright buildings in the back and the sky and lake colors. 
        }
        %vspace{-0.5cm}
		\label{fig:wu}
\end{figure}

